MDPs as Distribution Transformers: Affine Invariant Synthesis for Safety Objectives

Markov decision processes can be viewed as transformers of probability distributions. While this view is useful from a practical standpoint to reason about trajectories of distributions, basic reachability and safety problems are known to be computationally intractable (i.e., Skolem-hard) to solve in such models. Further, we show that even for simple examples of MDPs, strategies for safety objectives over distributions can require infinite memory and randomization. In light of this, we present a novel overapproximation approach to synthesize strategies in an MDP, such that a safety objective over the distributions is met. More precisely, we develop a new framework for template-based synthesis of certificates as affine distributional and inductive invariants for safety objectives in MDPs. We provide two algorithms within this framework. One can only synthesize memoryless strategies, but has relative completeness guarantees, while the other can synthesize general strategies. The runtime complexity of both algorithms is in PSPACE. We implement these algorithms and show that they can solve several non-trivial examples.

==> 0_macros.tex <==
\RequirePackage{xparse}


\newcommand{\expv}{\mathbb{E}}
\newcommand{\Eval}{\mathsf{ET}}
\newcommand{\Thr}{\mathsf{Thr}}

%\newcommand{\program}{P}
%
%\lstdefinelanguage{affprob}
%{
%	morekeywords={angel,demon, choice, prob, if, then, else, fi,
%		while, do, od,
%		true, false, and, or, skip, sample, assume, tick},
%	sensitive = false,
%	%	morecomment=[l]{//},
%	escapeinside={@:}{:@}
%}


\newcommand{\MC}{\mathsf{M}}
\newcommand{\MDP}{\mathcal{M}}
\newcommand{\States}{S}
\newcommand{\Actions}{\mathit{Act}}
\newcommand{\state}{s}
\newcommand{\action}{a}

\newcommand{\infinitepath}{\rho}
\newcommand{\finitepath}{\varrho}
\newcommand{\strategy}{\pi}
\newcommand{\Strategies}{\Pi}
\newcommand{\StrategiesMD}{\Strategies_\mathsf{MD}}
\newcommand{\StrategiesOS}{\Strategies_1}

\NewDocumentCommand{\IPaths}{d<>}{\IfValueTF{#1}{\mathsf{IPaths}_{#1}}{\mathsf{IPaths}}}
\NewDocumentCommand{\FPaths}{d<>}{\IfValueTF{#1}{\mathsf{FPaths}_{#1}}{\mathsf{FPaths}}}

\NewDocumentCommand{\ProbabilityMC}{s r<> d[]}{\mathsf{Pr}_{#2}\IfNoValueF{#3}{\IfBooleanTF{#1}{\!\left[#3\right]\!}{[#3]}}}

\DeclareMathOperator{\support}{supp}

\newcommand{\unionSym}{\cup}
\newcommand{\unionBin}{\mathbin{\unionSym}}
\newcommand{\strictunionSym}{\dot{\unionSym}}
\newcommand{\strictunionBin}{\mathbin{\dot{\unionSym}}}
\newcommand{\intersectionSym}{\cap}
\newcommand{\intersectionBin}{\mathbin{\intersectionSym}}
\newcommand{\UnionSym}{\bigcup}
\newcommand{\UnionBin}{\mathbin{\UnionSym}}
\newcommand{\strictUnionSym}{\dot{\UnionSym}}
\newcommand{\strictUnionBin}{\mathbin{\strictUnionSym}}
\newcommand{\IntersectionSym}{\bigcap}
\newcommand{\IntersectionBin}{\mathbin{\IntersectionSym}}

\newcommand{\union}{\unionBin}
\newcommand{\strictunion}{\strictunionBin}
\newcommand{\intersection}{\intersectionBin}
\newcommand{\Union}{\UnionSym}
\newcommand{\strictUnion}{\strictUnionSym}
\newcommand{\Intersection}{\IntersectionSym}

\newcommand{\Naturals}{\mathbb{N}}
\newcommand{\Reals}{\mathbb{R}}

\newcommand{\distribution}{\mu}
\NewDocumentCommand{\Distributions}{d()}{\IfNoValueTF{#1}{\Delta}{\Delta(#1)}}
\NewDocumentCommand{\Probability}{D[]{} D<>{} d[]}{
	\IfNoValueTF{#3}{\mathbb{P}_{#1}^{#2}}{\mathbb{P}_{#1}^{#2}\left[#3\right]}}
\NewDocumentCommand{\TS}{d<>}{\IfValueTF{#1}{\mathcal{T}_{#1}}{\mathcal{T}}}
\newcommand{\transitions}{\delta}
\newcommand{\act}{\mathsf{act}}


==> mdptoprogram.tex <==
\section{From MDPs to Programs}\label{sec:mdptoprograms}

We now show how each of the safety problems over probability distributions in MDPs in Section~\ref{sec:preliminaries} can be reduced to the problem of inductive invariant generation in programs. We start by presenting intuition behind the reduction and then proceed to formalizing the reduction details and proving reduction correctness. In what follows, we let $\MDP = (\States, \Actions, (M_\action)_{\action\in \Actions})$ be an MDP with $\States=\{\state_1,\dots,\state_n\}$ and $\Actions=\{\action_1,\dots,\action_m\}$. Let $H \subseteq [0,1]^n$ be a safe set specified by an intersection of $[0,1]^n$ and finitely many polynomial inequalities.

\smallskip\noindent{\bf Main idea behind the reduction} Recall, every strategy in $\MDP$ induces a sequence of probability distributions  $\Delta^0,\Delta^1,\dots \in [0,1]^n$ for every initial probability distribution $\Delta^0\in[0,1]^n$. We show that the process that generates $\Delta^0,\Delta^1, \dots$ can be written as an imperative program that consists of a single loop. The program has $n$ distinguished variables $x_1, \dots, x_n$, where each $x_i$ is used to capture the probability of the MDP being in state $\state_i$. To that end, each $x_i$ is initialized to the value of the $i$-th component of $\Delta^0$. The body of the loop is designed in a way that simulates the choice of the next action perscribed by some strategy and the application of the probability transformer induced by the strategy. Hence, the value of $x_i$ after $k$ loop iterations is equal to the probability of the MDP being in state $\state_i$ after $k$ steps, for each $1\leq i\leq n$ and $k\in\mathbb{N}_0$, so a strategy in the MDP is $H$-safe from some initial probability distribution if and only if the corresponding program that picks actions perscribed by the strategy never reaches a state with $(x_1,\dots,x_n)\not\in H$. In other words, a strategy in the MDP is $H$-safe from an initial probability distribution $\Delta^0$ if and only if the corresponding program admits a program invariant that is fully contained within $H$. Therefore, if we could design a method that synthesizes a strategy $\sigma$ together with a program invariant that witnesses that the strategy is $H$-safe, we can solve the safety problems defined in Section~\ref{sec:preliminaries}. In the rest of this section, we formalize the reduction and prove its correctness for each of the four safety problems.

\smallskip\noindent{\bf Program for safety under memoryless strategies} We start by formally describing the program construction in the case of each safety problem under memoryless strategies. The program to which each of the safety problems under memoryless strategies is reduced is shown in Fig.~\ref{fig:reductionmemoryless}. The program contains the following program variables:
\begin{compactitem}
	\item {\em Variables $x_i$.} For each $1 \leq i \leq n$, we introduce a program variable $x_i$ which is used to track the probability of the MDP being in state $\state_i$. In the case of the initialized safety problem, the values of $x_i$'s are initialized to the values of entries of the specified initial probability distribution $\Delta^0$. In the case of the existential safety problem, the values of $x_i$'s are initialized to some symbolic initial probability distribution $\Delta^0$ whose entry values are to be determined during the invariant synthesis. Finally, in the case of the universal safety problem, the values of $x_i$'s are initialized by non-deterministically picking an element of $H$ and assigning its entry values to $x_i$'s.
	
	\item {\em Variables $p_{\state_i, \action_j}$.}  Variable $p_{\state_i, \action_j}$ is used to encode the probability of picking action $\action_j$ at state $\state_i$ that is perscribed by a memoryless strategy, for each $1 \leq i \leq n$ and $1 \leq j \leq m$. Since we are interested in solving the safety problems with respect to memoryless strategies, the values of variables $p_{\state_i, \action_j}$ should only depend on the initial probability distribution $\Delta^0$ and not on subsequently generated probability distributions. Thus, in the case of memoryless strategies, the values of each $p_{\state_i, \action_j}$ are initialized {\em before} executing the loop and are {\em not modified} by the loop. The value of each $p_{\state_i, \action_j}$ is initialized to some symbolic value which is then to be determined during invariant synthesis, since our method jointly searches for the strategy and the invariant that witnesses $H$-safety under the strategy. We only restrict the values of $p_{\state_i, \action_j}$ to be contained in $[0,1]$ and to define probability distributions over the action space for each $\state_i$, which is encoded in the non-deterministic assignments that are used for the initialization in Fig.~\ref{fig:reductionmemoryless}.
	
	\item {\em Variables $x_i'$.} Finally, variables $x_i'$ are auxillary variables which are used to ensure that the updates of all $x_i$'s upon the execution of each loop iteration are performed simultaneously.
\end{compactitem}
The loop body simulates the application of the probability transformer induced by the strategy determined by values of program variables $p_{\state_i,\action_j}$. Given the values of $x_1,\dots,x_n$ which for each $1 \leq i \leq n$ encode the probability of the MDP being in a state $\state_i$ at a given time step, the loop body computes $x_1', \dots, x_n'$ as the probabilities of the MDP being in each $\state_i$ at the subsequent time step. We describe how this computation is performed for $x_1'$, as the computations for $x_2',\dots,x_n'$ are analogous. The probability of the MDP being in $\state_1$ in the subsequent step is equal to the sum over $i$ of the probability of the MDP currently being in $\state_i$ multiplied by the probability of moving from $\state_i$ to $\state_1$ in the subsequent step. This probability is equal to $\sum_{j=1}^m p_{s_i,a_j} \cdot M_{a_j}[s_i,s_1]$, since the probability of taking action $\action_j$ in $\state_i$ under the fixed memoryless strategy is $p_{\state_i,\action_j}$ and the probability of moving from $\state_i$ to $\state_1$ under action $\action_j$ is $M_{\action_j}[\state_i,\state_1]$, where $M_{\action_j}[\state_i,\state_1]$ is a scalar $(i,1)$-st entry of the stochastic matrix $M_{\action_j}$ in the MDP $\MDP$. Thus, multiplying each $x_i$ by this probability and taking the sum over all state indices $1 \leq i \leq n$, we obtain the expression for the update of $x_1'$ in Fig.~\ref{fig:reductionmemoryless}:
\[ x_1' = \sum_{i=1}^n \sum_{j=1}^m p_{s_i,a_j} \cdot M_{a_j}[s_i,s_1] \cdot x_i. \] 
Finally, the loop body updates the value of each $x_i$ to the value of $x_i'$, before proceeding to the next loop iteration. We set the loop guard to $(x_1,\dots,x_n) \in H$ so that the program terminates if and only if the MDP reaches a probability distribution over program states that is not contained in the safe set $H$.

\smallskip\noindent{\bf Program for safety under general strategies} We now describe the program construction in reduction from safety problems under general strategies. The program to which all three safety problems under general strategies are reduced is shown in Fig.~\ref{fig:reductiongeneral}. The construction of the program is analogous to the case of memoryless strategies in Fig.~\ref{fig:reductionmemoryless}, with the exception of how the values of program variables $p_{\state_i,\action_j}$ are initialized and updated. Recall, variables $p_{\state_i,\action_j}$ encode the probabilities of taking action $\action_j$ in state $\state_i$ under the fixed strategy in the MDP. Since we are now interested in solving the safety problems with respect to general strategies, the values of variables $p_{\state_i, \action_j}$ may {\em not only} depend on the initial probability distribution but {\em also} on the subsequently generated probability distributions. Thus, the values of each $p_{\state_i, \action_j}$ are now {\em updated} by non-deterministic assignments which are contained within the loop body.

\smallskip\noindent{\bf Inductive invariants in programs} \textcolor{blue}{Djordje: Define inductive invariants, focus on the special case of single-loop programs where we will only have invariants specified at the loop head.}

\smallskip\noindent{\bf From MDP safety to inductive invariant generation} \textcolor{blue}{Djordje: State and prove theorems on correctness of reductions and equivalence.}

\lstset{language=affprob}
\lstset{tabsize=2}
\newsavebox{\progmemoryless}
\begin{lrbox}{\progmemoryless}
	\centering
	\begin{lstlisting}[mathescape]
$(x_1, \dots, x_n) = \Delta^0$ OR $(x_1,\dots,x_n) = \textbf{ndet}(H)$
$(p_{s_1,a_1}, \dots, p_{s_1,a_m}) = \textbf{ndet}(0 \leq p_{s_1,a_1}, \dots, p_{s_1,a_m} \leq 1, p_{s_1,a_1} + \dots + p_{s_1,a_m} = 1)$
$\dots$
$(p_{s_n,a_1}, \dots, p_{s_n,a_m}) = \textbf{ndet}(0 \leq p_{s_n,a_1}, \dots, p_{s_n,a_m} \leq 1, p_{s_n,a_1} + \dots + p_{s_n,a_m} = 1)$
while $(x_1, \dots, x_n) \in H$ do
	$x_1' = \sum_{i=1}^n \sum_{j=1}^m p_{s_i,a_j} \cdot M_{a_j}[s_i,s_1] \cdot x_i$
	$\dots$
	$x_n' = \sum_{i=1}^n \sum_{j=1}^m p_{s_i,a_j} \cdot M_{a_j}[s_i,s_n] \cdot x_i$
	$(x_1, \dots, x_n) = (x_1', \dots, x_n')$
	\end{lstlisting}
\end{lrbox}

\begin{figure*}[t]
	\centering
	\usebox{\progmemoryless}
	%\caption{Running example. }
	%\label{fig:running}
	\caption{Program that encodes the existential OR universal safety problem under memoryless strategies. \textcolor{blue}{Djordje: To add details to caption.}}
	\label{fig:reductionmemoryless}
\end{figure*}

\lstset{language=affprob}
\lstset{tabsize=2}
\newsavebox{\programgeneral}
\begin{lrbox}{\programgeneral}
	\centering
	\begin{lstlisting}[mathescape]
$(x_1, \dots, x_n) = \Delta^0$ OR $(x_1,\dots,x_n) = \textbf{ndet}(H)$
while $(x_1, \dots, x_n) \in H$ do
	$(p_{s_1,a_1}, \dots, p_{s_1,a_m}) = \textbf{ndet}(0 \leq p_{s_1,a_1}, \dots, p_{s_1,a_m} \leq 1, p_{s_1,a_1} + \dots + p_{s_1,a_m} = 1)$
	$\dots$
	$(p_{s_n,a_1}, \dots, p_{s_n,a_m}) = \textbf{ndet}(0 \leq p_{s_n,a_1}, \dots, p_{s_n,a_m} \leq 1, p_{s_n,a_1} + \dots + p_{s_n,a_m} = 1)$
	$x_1' = \sum_{i=1}^n \sum_{j=1}^m p_{s_i,a_j} \cdot M_{a_j}[s_i,s_1] \cdot x_i$
	$\dots$
	$x_n' = \sum_{i=1}^n \sum_{j=1}^m p_{s_i,a_j} \cdot M_{a_j}[s_i,s_n] \cdot x_i$
	$(x_1, \dots, x_n) = (x_1', \dots, x_n')$
	\end{lstlisting}
\end{lrbox}

\begin{figure*}[t]
	\centering
	\usebox{\programgeneral}
	%\caption{Running example. }
	%\label{fig:running}
	\caption{The program that encodes the existential OR universal safety problem under general strategies. \textcolor{blue}{Djordje: To add details to caption.}}
	\label{fig:reductiongeneral}
\end{figure*}

\section{Inductive Invariant Synthesis with Strategy Search}\label{invariantsynthesis}

We now present our algorithm for safety analysis in MDPs by reduction to inductive invariant synthesis in programs. To simplify the presentation, we start by presenting our algorithm for the initialized and uninitialized safety problems under memoryless strategies. We then show how our algorithm extends to the case of the initialized and uninitialized safety problems under general strategies.

\smallskip\noindent{\bf Algorithm input.} The algorithm takes as input an MDP $\MDP = (\States, \Actions, (M_\action)_{\action\in \Actions})$ with $\States = \{\state_1,\dots,\state_n\}$ and $\Actions = \{\action_1,\dots,\action_m\}$, as well as a safety set $H \subseteq [0,1]^n$ defined as an intersection of $[0,1]^n$ and finitely many strict or non-strict polynomial inequalities. In addition, for the initialized safety problem, it also takes as input an initial probability distribution $\Delta^0\in[0,1]^n$. The algorithm also takes as input technical parameters \textcolor{blue}{Djordje: List of all parameters}, which specify polynomial template size to be used. These will be formally defined shortly. 

%We present two algorithms. The first algorithm is applicable to the case when $H$ is specified in terms of strict or non-strict {\em affine} inequalites and it searches for the strategy and an inductive invariant specified in terms of {\em non-linear affine inequalities}. The second algorithm is applicable to the more general setting when $H$ is specified in terms of strict or non-strict {\em polynomial inequalities} and it searches for the strategy and an inductive invariant specified in terms of {\em strongly positive polynomial inequalities} (a notion which we define later in this section). The reason why we present both algorithms is that the first algorithm provides stronger completeness guarantees, whereas the second algorithm is applicable to the more general setting of polynomial safety sets.

\smallskip\noindent{\bf Algorithm output.} The algorithm first translates the safety problem at hand to the program $P$ in Fig.~\ref{fig:reductionmemoryless}. In Section~\ref{sec:mdptoprograms}, we showed that this program simulates an MDP probability distribution transformer under memoryless strategies. The algorithm then computes the values of parameters $p_{\state_i,\action_j}$ and a predicate $I$ so that the values of $p_{\state_i,\action_j}$'s define a strategy in $\MDP$ and $I$ defines an inductive invariant with respect to these values of $p_{\state_i,\action_j}$'s and the initial values of $x_1,\dots,x_n$ specified by $\Delta^0$. The predicate $I$ is computed as a conjunction of finitely many strongly positive polynomial inequalities over the variable set $\{x_1,\dots,x_n\}$. In the case of the uninitialized safety problem, the algorithm also computes $n$ real values to determine the initial probability distribution $\Delta^0$.

\smallskip\noindent{\bf Algorithm outline.} Our algorithm employs a template-based approach to simultaneously synthesize polynomial expressions that determine $p_{\state_i,\action_j}$'s and $I$, as well as the concrete values for $\Delta^0$ in the case of the uninitialized safety problem. Given the program $P$, it proceeds in four steps:
\begin{compactenum}
	\item {\em Setting up templates.} The algorithm fixes a symbolic polynomial expression for each $p_{\state_i,\action_j}$, a symbolic polynomial template for $I$ and symbolic values for the initial probability distribution $\Delta^0$, if necessary. Note that the values of symbolic template variables are {\em unknown} at this point and are to be computed in subsequent steps. 
	\item The algorithm collects the constraints that encode that $I$ contains the initial probability distribution $\Delta^0$, that $I$ is an inductive invariant with respect to the values of $p_{\state_i,\action_j}$ defined by the symbolic template and that $I$ is contained within $H$. This step yields a system of polynomial constraints over symbolic template variables that contain both universal and existential quantifiers.
	\item {\em Quantifier elimination.} The algorithm now elimintates universal quantifiers from the above to reduce it to a system of purely existentially quantified system of constraints over the symbolic template variables.
	\item {\em Constraint solving.} By using an off-the-shelf solver, the algorithm solver the resulting system of existentially quantified polynomial constraints over the symbolic template variables to compute the concrete values of coefficients in the expressions for  each $p_{\state_i,\action_j}$ and $I$ and the concrete values of $\Delta^0$. 
\end{compactenum}

\smallskip\noindent{\bf Algorithm novelty.} Note that the template-based synthesis is a standard approach to invariant synthesis in programs~\cite{xxx}. However, the key conceptual novelty of our algorithm that we synthesize the invariant {\em jointly} with the values of $p_{\state_i,\action_j}$'s that define a strategy in the MDP.

\smallskip In what follows, we describe each of the four steps in detail.

\smallskip\noindent{\bf Step~1: Setting up templates.} 

\smallskip\noindent{\bf Step~2: Constraint collection.} 

\smallskip\noindent{\bf Step~3: Quantifier elimination.} 

\smallskip\noindent{\bf Step~4: Constraint solving.} 


It then computes the following two or three objects, depending on whether we are considering the initialized or the uninitialized safety problem:
\begin{enumerate}
	\item {\em Initial probability distribution $\Delta^0$.} In the case of the initialized safety problem, $\Delta^0$ is already provided as part of the input. Otherwise, the algorithm 
	\item {\em Strategy $\sigma$.}
	\item {\em Inductive invariant $I$.}
\end{enumerate}
